Bilevel methods for image reconstruction

This review discusses methods for learning parameters for image reconstruction problems using bilevel formulations. Image reconstruction typically involves optimizing a cost function to recover a vector of unknown variables that agrees with collected measurements and prior assumptions. State-of-the-art image reconstruction methods learn these prior assumptions from training data using various machine learning techniques, such as bilevel methods. One can view the bilevel problem as formalizing hyperparameter optimization, as bridging machine learning and cost function based optimization methods, or as a method to learn variables best suited to a specific task. More formally, bilevel problems attempt to minimize an upper-level loss function, where variables in the upper-level loss function are themselves minimizers of a lower-level cost function. This review contains a running example problem of learning tuning parameters and the coefficients for sparsifying filters used in a regularizer. Such filters generalize the popular total variation regularization method, and learned filters are closely related to convolutional neural networks approaches that are rapidly gaining in popularity. Here, the lower-level problem is to reconstruct an image using a regularizer with learned sparsifying filters; the corresponding upper-level optimization problem involves a measure of reconstructed image quality based on training data. This review discusses multiple perspectives to motivate the use of bilevel methods and to make them more easily accessible to different audiences. We then turn to ways to optimize the bilevel problem, providing pros and cons of the variety of proposed approaches. Finally we overview bilevel applications in image reconstruction.

==> NOWFnT-data.tex <==
\newcommand\nowfnt@publicationaddress
 {%
  \textit{Published, sold and distributed by:}\\
  now Publishers Inc.\\
  PO Box 1024\\
  Hanover, MA 02339\\
  United States\\
  Tel.\ +1-781-985-4510\\
  www.nowpublishers.com\\
  sales@nowpublishers.com%
  \par
  \textit{Outside North America:}\\
  now Publishers Inc.\\
  PO Box 179\\
  2600 AD Delft\\
  The Netherlands\\
  Tel.\ +31-6-51115274
 }

\newcommand\nowfnt@legalrightstext
 {%
  All rights reserved. No part of this publication may be
  reproduced, stored in a retrieval system, or transmitted in any form or by any means, mechanical, photocopying, recording or otherwise, without prior written permission of the publishers.
  \par
  Photocopying. In the USA: This journal is registered at the Copyright  Clearance Center, Inc., 222 Rosewood Drive, Danvers, MA 01923.  Authorization to photocopy items for
  internal or personal use, or the internal or personal use of specific  clients, is granted by now Publishers Inc for users registered with the Copyright Clearance Center (CCC).
  The `services' for users can be found on the internet at:
  www.copyright.com
  \par
  For those organizations that have been granted a photocopy license, a separate system of payment has been arranged. Authorization does not extend to other kinds of copying, such as that for general distribution, for advertising or promotional purposes, for creating new collective works, or for resale.  In the rest of the world:
  Permission to photocopy must be obtained from the copyright
  owner. Please apply to now Publishers Inc., PO Box 1024, Hanover, MA 02339, USA; Tel. +1 781 871 0245; www.nowpublishers.com; sales@nowpublishers.com
  \par
  now Publishers Inc. has an exclusive license to publish this
  material worldwide. Permission to use this content must be obtained from the copyright license holder. Please apply to now Publishers, PO Box 179, 2600
  AD Delft, The Netherlands, www.nowpublishers.com; e-mail:
  sales@nowpublishers.com}

\newcommand\nowfnt@printedoninfotext
 {%
  {%
   %
  }%
 }

\newcommand\nowfnt@howtocitetext
 {%
  The preferred citation for this publication is\par
  {%
   \raggedright
   \useissuedata{copyrightowner}.
   \emph{\nowfnt@articletitle}.
   \printjournaltitleprefix \usejournaldata{title}, vol.~\useissuedata{volume}, no.~\useissuedata{issue}, pp.~\useissuedata{firstpage}--\useissuedata{lastpage},
   \useissuedata{pubyear}.%
  }%
 }


\newcommand\nowfnt@copyrightlinetext
 {%
  ISBN: \useissuedata{isbn}\\
  \copyright\ \useissuedata{copyrightyear} \useissuedata{copyrightowner}}

\newcommand\nowfnt@NOWcopyrightlinetext  %for wrapper
  {%
  ISBN: \useissuedata{isbn}\\
  \copyright\ \useissuedata{copyrightyear} Now Publishers Inc}

\newcommand\nowfnt@sourceintro{%
 The content of the book was originally published in  }

\newcommand\nowfnt@sourcepunct{.}

\newcommand\nowfnt@prohibitiontext{This article may be used only for the purpose of research, teaching, and/or private study. Commercial use or systematic downloading (by robots or other automatic processes) is prohibited without explicit Publisher approval.}

\newcommand\nowfntstandardcitation{\nowfnt@authorlist@toc\ (\nowfnt@issuepubyear), \enquote{\nowfnt@articletitle}, \nowfnt@journaltitle: Vol. \nowfnt@issuevolume, No. \nowfnt@issueissue, pp \nowfnt@issuefirstpage--\nowfnt@issuelastpage. DOI: \nowfnt@issuedoi.}

%Title for the series pages.
\newcommand\nowfnt@seriespagetitle{\section*{Other titles in \nowfnt@journaltitle}}

==> SIG-journaldata.tex <==
 \definecolor{palatinapurple}{rgb}{0.41, 0.16, 0.38}
\colorlet{SIGcolor}{palatinapurple}   %new color names can be defined before use
\journalcolor      {SIGcolor} %a color name.
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Signal Processing}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {SIG}
\journalurl        {http://www.nowpublishers.com/SIG}
\journalissnprint  {1932-8346}
\journalissnonline {1932-8354}
\journaldoi        {10.1561/20}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{numeric} % either author or numeric

\journalaimsandscope
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Signal Processing publishes
 survey and tutorial articles in the following topics:
 \begin{multicols}{2}\raggedcolumns
\footnotesize
 \begin{itemize}
\item{Adaptive signal processing}
\item{Audio signal processing}
\item{Biological and biomedical signal processing}
\item{Complexity in signal processing}
\item{Digital signal processing}
\item{Distributed and network signal processing}
\item{Image and video processing}
\item{Linear and nonlinear filtering}
\item{Multidimensional signal processing}
\item{Multimodal signal processing}
\item{Multirate signal processing}
\item{Multiresolution signal processing}
\item{Nonlinear signal processing}
\item{Randomized algorithms in signal processing}
\item{Sensor and multiple source signal processing, source separation}
\item{Signal decompositions, subband and transform methods, sparse representations}
\item{Signal processing for communications}
\item{Signal processing for security and forensic analysis, biometric signal processing}
\item{Signal quantization, sampling, analog-to-digital conversion, coding and compression}
\item{Signal reconstruction, digital-to-analog conversion, enhancement, decoding and inverse problems}
\item{Speech/audio/image/video compression}
\item{Speech and spoken language processing}
\item{Statistical/machine learning}
\item{Statistical signal processing}
	\begin{itemize}
	\item{Classification and detection}
	\item{Estimation and regression}
	\item{Tree-structured methods}
	\end{itemize}
\end{itemize}
\normalsize
 \end{multicols}
 }


\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Signal Processing, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 }


==> TablesAndAlgs/tab,summary,methods.tex <==
% not used 

\begin{table}[htbp]
    \centering
    \begin{tabular}{p{1.5cm}|p{2.cm}|p{1.5cm}|p{1.5cm}|p{1.8cm}|p{2.7cm}}
        Paper & 
            $R(\vx)$ & Upper-level & \params & 
            Opt. approach (LL/UL) & Application\\ \hline 
        \textcite{peyre:2011:learninganalysissparsity} & 
            $\sparsefcn(\mC \vx)$, \sparsefcn is CR1N & MSE & Filter coefficients & 
            ?/GD & 1d denoising \\ \hline
        \textcite{chen:2014:insightsanalysisoperator} &
            $\sum_k \ebeta{k} \sparsefcn(\mC_k \vx)$, multiple \sparsefcn & MSE & Linear coefficients for filter basis and $\beta_k$ & 
            L-BFGS/L-BFGS & Image denoising*\\ \hline
        \textcite{holler:2018:bilevelapproachparameter} & 
            $\beta \sum_k \sparsefcn(\mC_k \vx)$ (more generic for theory, 2-norm \sparsefcn with identity and differential $\mC_k$'s for results) & MSE & Tuning parameter, $\beta$ & 
            \todo{not sure for the first application} or sequential programming method/BFGS & Two second order elliptic PDEs \\ \hline
        \textcite{fehrenbach:2015:bilevelimagedenoising} & 
            $\sum_k \ebeta{k} \sparsefcn(\mC_k \vx)$, \sparsefcn is CR1N & Gaussianity of noise in frequency partitions & $\beta_k$ & 
            Accelerated proximal GD on dual problem/Gauss-Newton alg. & Image denoising \\ \hline
        \textcite{holler:2018:bilevelapproachparameter} &
            & $\sum_k \beta_k \sparsefcn(\mC_k \vx)$, \sparsefcn is squared 2-norm & MSE & $\beta_k$
            & Varies/BFGS with line search \\ \hline
    \end{tabular}
    \caption{IFT}
    \label{tab: example ift papers}
\end{table}


\begin{table}[h]
    \centering
    \begin{tabular}{p{1.5cm}|p{2.cm}|p{1.5cm}|p{1.5cm}|p{1.8cm}|p{2.7cm}}
        Paper & 
            $R(\vx)$ & Upper-level & \params & 
            Opt. approach (LL/UL) & Application\\ \hline 
        \textcite{antil:2020:bileveloptimizationdeep}&
            The norm of the Fractional Laplacian applied to \vx & MSE & Fractional Laplacian power, $\beta$
            & Both: Projected GD with line search & \\ \hline
        \textcite{chen:2020:learnabledescentalgorithm} &
            Deep neural network & MSE & DNN weights & 
            Modified GD/Adam & Compressed sensing, Joint compression and reconstruction, MRI reconstruction\\ \hline
        &
            & & & 
            & \\ \hline
    \end{tabular}
    \caption{Unrolled}
    \label{tab: example unrolled papers}
\end{table}

\todo{Notes to myself to put somewhere or fix:} 
\begin{itemize}[noitemsep]
    \item CR1N = corner rounded 1-norm (don't think we need to detail how they round the corner) 
    \item Note some of the papers write the regularization more generally for an analysis operator that is a matrix, but I've written them as convolutions if that is the bulk of the presentation of the paper 
    \item *\textcite{chen:2014:insightsanalysisoperator} also does image deconvolution, super-resolution, inpainting, but they do not learn new filters, just apply the ones from the denoising bilevel set-up 
\end{itemize}
